Immersion on the Edge: A Cooperative Framework for Mobile Immersive Computing

Immersive computing (IC) technologies such as virtual reality and augmented reality are gaining tremendous popularity. In this poster, we present CoIC, a Cooperative framework for mobile Immersive Computing. The design of CoIC is based on a key insight that IC tasks among different applications or users might be similar or redundant. CoIC enhances the performance of mobile IC applications by caching and sharing computation-intensive IC results on the edge. Our preliminary evaluation results on an AR application show that CoIC can reduce the recognition and rendering latency by up to 52.28% and 75.86% respectively on current mobile devices.

==> abstract.tex <==
\begin{abstract}

    %Immersive computing (IC) technologies such as virtual reality and augmented reality are gaining tremendous popularity.
    %Mobile IC applications are changing the way people interact with mobile devices. End-to-end latency is the key QoE metric for IC applications.
    %In this poster, 
    We present \name, a \textbf{Co}operative framework for mobile \textbf{I}mmersive \textbf{C}omputing. The design of \name is based on a key insight that IC tasks among different applications or users might be similar or redundant. \name enhances the performance of mobile IC applications by caching and sharing computation-intensive IC results on the edge.
    Our preliminary evaluation results on an AR application show that \name can reduce the recognition and rendering latency by up to 52.28\% and 75.86\% respectively on current mobile devices.

\end{abstract}


==> conclusion.tex <==
\section{Conclusion}

==> implementation.tex <==
\section{Implementation}

We implemented \cosar upon TensorFlow Lite on a Pixel smartphone running Android O.

==> introduction.tex <==
\section{Introduction}

==> motivation.tex <==
\section{Motivation}


Accomplishing the above three QoE requirements simutaneously for high-quality social AR apps has remained unattainable on today's mobile devices due to the limited capability of mobile hardware and wireless technologies. In this section we conducted a series of experiments to investigate the performance issue existing in the state-of-the-art social AR systems and explain the root cause.



\subsection{Accomplishing low latency and high accuracy simutaneously is challenging}


We first conduct an experiment to measure the achievable frame processing latency and accuracy of social AR systems on today's mobile devices. Specifically, we implement a social AR protoype based on TensorFlow Lite. The prototype leverages classic machine learning model (e.g. DNN) for object recognition. We run the AR prototype on a Pixel smartphone running Android O. We manually adjust the recognition interval and measure the per-frame processing latency to gether with the recognition latency.

Figure X plots the measurement results.


Data.

Root cause.

Drawback of existing systems: (1) high latency? (2) low-quality? (3) low accuracy?

Root cause analysis: constrained computation capability.

Key insights: (1) frame flow; (2) control flow; (3) rendering flow;


\subsection{Rendering high-quality 3D annotations in high framerate is challenging}

Next we conduct an experiment to measure the rendering overhead. Typically, in a social AR system the render engine renders a 3D annotation based on recognition results and user interactions. 

Data.

Root cause.









